Improving Limited Supervised Foot Ulcer Segmentation Using Cross-Domain Augmentation

Diabetic foot ulcers pose health risks, including higher morbidity, mortality, and amputation rates. Monitoring wound areas is crucial for proper care, but manual segmentation is subjective due to complex wound features and background variation. Expert annotations are costly and time-intensive, thus hampering large dataset creation. Existing segmentation models relying on extensive annotations are impractical in real-world scenarios with limited annotated data. In this paper, we propose a cross-domain augmentation method named TransMix that combines Augmented Global Pre-training AGP and Localized CutMix Fine-tuning LCF to enrich wound segmentation data for model learning. TransMix can effectively improve the foot ulcer segmentation model training by leveraging other dermatology datasets not on ulcer skins or wounds. AGP effectively increases the overall image variability, while LCF increases the diversity of wound regions. Experimental results show that TransMix increases the variability of wound regions and substantially improves the Dice score for models trained with only 40 annotated images under various proportions.

==> rebuttal_old.tex <==
``The methodology presented in the paper, particularly the
use of cross-domain data for machine learning in medical
applications, has the potential for adaptation and
application in other areas of medical image analysis,
indicating its broader relevance in the field.''


GPU info: nVidia Quadro RTX 6000/8000
Batch size: 4
Epoch: 300
Training 40 time: 3.2~3.5 sec/epoch, 6 sec/epoch
Training 40 memory: 5.39 GB
Training 81 time: 3.61 GB
Training 81 memory: 4.99 GB
Inference time: 5~7 sec/200 images
Inference memory: 1.16 GB (batch size=4) 


Our method works with public and specific domain data. Rapid fine-tuning using a shared pre-trained model enables effective model transfer to new targets.

R3-5: Expanding on the real-world applicability and any practical challenges in clinical implementation would provide a more comprehensive understanding of the method’s utility.

A: We appreciate the reviewer's suggestions. Please refer to the responses in R1-1 and R2-3.


Wound segmentation in medical images allows precise assessment, efficient monitoring, and personalized treatment, enhancing healthcare outcomes. Training models for specific biomedical tasks usually demands a large annotated dataset. However, real-world medical applications face challenges in image data collection due to the privacy, ethical, and legal constraints, as well as variability in imaging protocols and patient recruitment. Medical image annotation is also challenging and costly, requiring specialized expertise and time. Training high-performing models with limited data can address the challenge of data scarcity and significantly assist the medical field.

==> sections/Experiment.tex <==



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Experimental setup}


% introduce the training parameters(e.g. lr, epochs, optimizer...) and dataset
% We adopt a widely used large-scale benchmark HAM10000\cite{ham10000} as our pre-training dataset, It consists of 10,015 skin lesion and mask image pairs, which are used to transfer the information to the foot ulcer segmentation task, and then we use FUSeg\cite{fuseg} dataset as our training and evaluation dataset, it has 810 foot ulcer image and mask pairs. In our experiments, we randomly sampled a portion of the data to simulate scenarios with limited data, utilizing proportions of 5\%, 10\%, 25\%, 50\%, and 100\%. We employed the U-Net model as our segmentation model and used Adam optimizer with 5e-4 learning rate, and training with 300 epochs and batch size of 4, the learning rate is decayed by a factor of 10 every 100 epochs.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsubsection{Compared Models}

% To achieve cross-domain transfer learning and increase data diversity for wound segmentation tasks, we compared the performance of pre-training and augmented global pre-training to validate the effectiveness of narrowing the domain gap. Additionally, we conducted experiments to assess the impact of random pasting during CutMix and whether background removal was performed, and we present the results in Table~\ref{table:main_results}.



% \textcolor{green}{
% \begin{itemize}
%     \item U-Net: 
%     \item Pre: 
%     \item GT
%     \item Cutmix
%     \item BT
% \end{itemize}
% }


% (Po-han: if implementation details too long, could simplify to below)
%We adopt a widely used large-scale benchmark HAM10000 as our pre-training dataset, It consists of 10,015 skin lesion and mask image pairs, which are used to transfer the information to the foot ulcer segmentation task, and then we use FUSeg dataset as our training and evaluation dataset, it has 810 foot ulcer image and mask pairs. In our experiments, we randomly sampled a portion of the data to simulate scenarios with limited data, utilizing proportions of 5\%, and 10\%. We employed the U-Net model as our segmentation model and used Adam optimizer with 5e-4 learning rate, and training with 300 epochs and batch size of 4, the learning rate is decayed by a factor of 10 every 100 epochs.


==> sections/Introduction.tex <==


%Foot ulcers, a prevalent complication of diabetes, contribute significantly to morbidity, mortality, and the risk of lower leg amputations, presenting a substantial public health challenge~\cite{DFU_2021}. Segmenting wound regions is essential to managing wound conditions and monitoring the healing trajectory. Manual segmentation depends on strong expertise and experience owing to highly varied etiologies and wound visual appearances. The resulting time-consuming and subjective segmentation process imposes immense burdens on clinical practice, intensifying the critical need for an automatic segmentation model.


%The automation of wound label segmentation is indispensable for expediting diagnoses and guiding treatment decisions. 
%\textcolor{purple}{(Jacob: No need to mention "automation" in the previous sentence? Just say segmentation is important.)}
%However, manual segmentation imposes resource, expertise, and bias-related burdens~\cite{ramachandram2022fully}, intensifying the critical need for an automatic segmentation model development.



%These model designs and ensemble strategies solely adjust the network architectures without any manipulations on raw image space which still hinders the learning for diverse wound types. The over-parameterized models can even fail to capture the wound patterns as there are only limited labeled training data accessible~\cite{limited_data_2017}. 


%Benefiting from the advancements in deep learning technology, convolutional models have shown impressive accuracy in image segmentation tasks. Most related research has focused on fine-tuning model architectures in pursuit of improved performance. Automatic Segmentation~\cite{automatic_segmentation}, for instance, builds upon Mask R-CNN~\cite{mask_rcnn}, enhancing it by incorporating a segmentation head for mask prediction. Some studies~\cite{fuseg_challenge_2, ensemble} also employ ensemble techniques by combining predictions from several model architectures, resulting in more stable and accurate results.
%LightWeight~\cite{lightweight} takes a different approach by utilizing residual attention and transforming inputs into patches to pay closer attention to local details, consequently enhancing overall performance.
%FUSegNet~\cite{fugsegnet_challenge_1}, on the other hand, refines the U-Net~\cite{unet} architecture by integrating spatial and channel squeeze-and-excitation modules during the decoding phase. By ensembling five models' results, it achieves state-of-the-art performance.
%\textcolor{purple}{(Jacob: It would be better to mention "however, the above works cannot perform well with limited data..." here. It would be better if we could find a citation. If not, say "as will be shown in our experiments".)}



% Past cross-domain research in the field of medical images attempts to address the issue of data scarcity by designing adaptation strategies. 
% 
%, has sought to design . This research primarily concentrates on various data sources that pertain to the same set of labeled classes.
%However, existing research has not taken into account the impact of limited data, considering the increasing cost of annotating new data in the future. 
%Zhou et al. extend diabetic retinopathy to recognizing multiple ocular diseases and extend glioma identification to the diagnosis of other brain tumors~\cite{zhou2021cct}

%We conducted an in-depth study on the relationship between data volume and model accuracy using the FUSeg~\cite{fuseg} dataset and found that when we only used 80 images for training data, the model's accuracy was lower compared to using 810 images.
%\textcolor{purple}{(Jacob: The previous sentence can be moved into the next (the 4th) paragraph. The 3rd paragraph can start with the following sentence, but avoid such a word "some". We can first say "transfer learning" is an effective way to alleviate the data scarcity issue, however, existing works focused on "domain adaptation", which is not applicable in our case... After that, use a new (the 4th) paragraph to describe our strategy.)}
%Some studies have attempted to address the issue of data scarcity by employing domain adaptation, where training is conducted with data from a similar domain and the same class to mitigate the decline in accuracy.
%As mentioned above, obtaining publicly available wound image segmentation datasets can be challenging. 


%We also conduct ablation studies and provide insights into the effects of global knowledge transfer and localized wound augmentation.

%Therefore, we opted for transfer learning using the HAM10000~\cite{ham10000, ham10000_mask} dataset, which has a skin lesion domain but different segmentation objectives. Due to its relatively uniform shooting angles and lower shape diversity, using it as a direct pretraining dataset would actually decrease the model's performance. To overcome this, we applied various data augmentation techniques (e.g., GridDistortion, Perspective, OpticalDistortion, etc.) to deform the HAM10000 data, making it more consistent with the segmentation objectives of the FUSeg dataset. This approach allows us to achieve the goal of global transfer for segmentation.
% However, existing research has not taken into account the impact of limited data, considering the increasing cost of annotating new data in the future. We conducted an in-depth study on the relationship between data volume and model accuracy and found that when we use only 80 images as training data, the model shows poor accuracy compared with using 810 images. 

% Some works tried to use domain adaptation to solve limited data issue, since they use similar domain's data to learn the target label information,
% (other use domain adaptation, but why we didn't use this method)
% (Classical Domain adaptation why can't, e.g. cause most of them is same target label but different feature)

% Therefore, we propose cross-domain augmentation to bridge different domains of labeled data (e.g., HAM10000~\cite{ham10000, ham10000_mask}) using specific augmentations, aiming to enhance the model's performance when data is scarce.
% (Why global transfer? observe and solution)


%Additionally, to further diversify the representation of wound regions, we use mixup series method to synthesize the image. Some studies~\cite{mixup, cutmix, cutout} have shown that such operations can significantly improve the model's generalization capabilities, while these methods ignore the region consistency and the localize ability, which is important for the wound segmentation task. Therefore, we proposed TransMix, which apply cutmix on different wound region, to ensure the wound area and background's consistency. Through this method, we increase the wound appearance diversity within limited labeled data to improve the model's performance.
% (localize ability, background consistency, first augmented then mix, while these method ....)
% intensifying the critical need for an accurate segmentation model developed with limited labeled data.


% To address this pressing issue, we present a novel approach that initially harnesses a cross-domain dataset for pre-training to impart fundamental segmentation capabilities and enhance wound variability in our model. We then introduce the proposed wound-mix technique, complemented by well-designed augmentation strategies, to fine-tune our model on the target dataset while further augmenting wound variability. This multifaceted approach empowers our model to precisely segment foot ulcers within a substantial testing dataset, all while training with a limited set of labeled data.



% Our method attains remarkable results on the FUSeg dataset, achieving a Dice score of X, marking a substantial improvement over the baseline models trained via conventional methods. These findings not only highlight the promise of our approach but also offer significant potential for advancing diabetes-related wound care. By bridging the gap between labor-intensive manual segmentation and the imperative for efficient, automated segmentation in clinical practice, our method has the potential to enhance patient outcomes and streamline healthcare processes.

% %%% State the importance of foot ulcer segmentation
% The segmentation problem of foot ulcers has been gaining attention as the number of diabetes patients rises. However, due to the need for medical professionals with specialized knowledge to annotate image masks, the annotation process is time-consuming and costly. This high annotation cost results in a scarcity of data compared to more common publicly available datasets. Even though there have been significant advances in deep learning techniques, the limited amount of data often hinders the training of models with high accuracy and generalization capabilities.


%%% Automatic segmentation is essential due to wound variability and assessment subjectivity (a few previous works done)
% \textcolor{red}{Wound images encompass substantial visual appearance variability which leads to considerable inter-rater variability and biased clinical decisions~\cite{ramachandram2022fully}.} % 4 different tissue types (epithelial, granulation, slough, and eschar), other variability might due to skin tones





%%% Limited data causes severe problems and thus other medical image studies have explored a few. Seldom of them have worked on wounds. With less data, the diversity of wound types and stages becomes difficult to learn.


%%% Therefore, we propose a xx-mix strategy to augment the variability with very few supervised samples ...



% \subsection{Related part}
% First introduce previous method used in FUSeg(MICCAI 2021 challendge) ~3 paper.

% Second introduce classical segmentation model(e.g. U-Net, PSPNet, DeepLabV3 ...).

% Third introduce the Cutmix series paper(Mixup, Cutmix, Cutout ...)



==> sections/Method.tex <==

% \begin{table*}[t]
% \begin{center}
% \caption{We conducted experiments on the proposed augmented global pre-training and localized CutMix techniques using the FUSeg dataset and reported their precision, recall, and dice scores.}
% \label{table:main_results}
% \begin{tabular}{l|cccccc}
% \hline
% \multicolumn{1}{c|}{\multirow{3}{*}{Model}} & \multicolumn{6}{c}{\# Sample} \\ \cline{2-7} 
% \multicolumn{1}{c|}{} & \multicolumn{3}{c|}{40(5\%)} & \multicolumn{3}{c}{81(10\%)} \\ \cline{2-7} 
% \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{Precision(\%)} & \multicolumn{1}{c|}{Recall(\%)} & \multicolumn{1}{c|}{Dice(\%)} & \multicolumn{1}{c|}{Precision(\%)} & \multicolumn{1}{c|}{Recall(\%)} & Dice(\%) \\ \hline
% U-Net & \multicolumn{1}{c|}{67.99} & \multicolumn{1}{c|}{83.18} & \multicolumn{1}{c|}{74.83} & \multicolumn{1}{c|}{86.98} & \multicolumn{1}{c|}{73.24} & 79.52 \\ \hline
% + Pretrain & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{66.03} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & 75.87 \\ \hline
% + Global Transfer & \multicolumn{1}{c|}{84.99} & \multicolumn{1}{c|}{79.60} & \multicolumn{1}{c|}{82.21} & \multicolumn{1}{c|}{84.87} & \multicolumn{1}{c|}{86.50} & 85.68 \\ \hline
% + Cutmix & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & - \\ \hline
% + Background Removed & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & - \\ \hline
% + Localize Cutmix & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & - \\ \hline
% + TransMix & \multicolumn{1}{c|}{82.50} & \multicolumn{1}{c|}{88.22} & \multicolumn{1}{c|}{85.26} & \multicolumn{1}{c|}{84.83} & \multicolumn{1}{c|}{88.51} & 86.65 \\ \hline
% \end{tabular}
% \end{center}
% \end{table*}


%Fig.~\ref{fig_framework} shows the architecture of our cross-domain augmentation strategies, which are composed of global transfer and localized augmentation. We first introduce the pre-training method and augmentation strategies of global transfer in $\S$\ref{sssec:global_transfer}. Then we introduce our localized mixup augmentation method in $\S$\ref{sssec:localized_augmentation}.
% In further detail, global transfer. Following this phase, we fine-tune the model on a restricted subset of the FUSeg dataset, employing augmentation and leveraging the self-cutmix skill to further enhance performance.


% \subsection{Dataset}
% Introduce HAM100000 and FUSeg dataset
% \textcolor{purple}{(Jacob: move to Experiment)}


% \textcolor{purple}{
% To evaluate the effectiveness of our framework in  In our experiments, we randomly sample 5\%, 10\%, 25\%, and 50\% of data and obtain subsets of different sizes 40, 80, 200, and 400 as the training data available in data-scarce scenarios. To extract skin-related global knowledge, we adopt the widely-used large-scale HAM10000 dataset~\cite{{ham10000}}, which consists of 10,015 skin lesion images along with their ground-truth masks. (Implementation details, including baseline methods and all the abbreviations such as U-Net, Pre, GT, Cutmix, BT, and LC).}

%we aim to transfer the acquired global skin related knowledge into the FUSeg dataset with intense augmentation strategies. In addition, we also propose a location-aware mixup technique to enhance the wound variability to further improve model performance. We detail each step in the following sections.}

%In the global transfer stage, due to the limited available data of the target FUSeg dataset, we pre-train our model on the HAM10000 dataset for establishing a foundational capability of wound segmentation. Then we fine-tune our model on the FUSeg dataset.\\



%Therefore, unlike the general pre-training policy that aims to train a high-performance model on their pre-train dataset, we regard alignment with the target dataset as our foremost consideration in pre-training our model. 
%In further detail, we perform strong spatial-level transformations such as affine, optical distortion, and perspective transformations to align photograph angles with the FUSeg dataset. Also, we perform strong pixel-level transformations such as RGB shift, brightness contrast, and hue saturation value transformations to align illumination conditions with the FUSeg dataset.\\
%\textcolor{purple}{As shown in Fig.~\ref{fig_framework}, images in the HAM10000 dataset exhibit highly consistent camera position and angle, whereas FUSeg contains images captured under various}







%In addition to the observations mentioned above, we also noticed a significant variability in wound characteristics within the FUSeg dataset. The global transformation method can augment the variation of shooting perspective and color tone. However, global transformation cannot increase the variability of the wound in the images. Thus, to further increase the wound variability using the limited data, we propose an augmentation method, TransMix, that can greatly enhance the diversity of wound characteristics and further boost the performance of our model by only using a limited amount of data.
%Generally speaking, TransMix is a method that pastes a ramdomly chosen wound patch on images during training to allow for more variation in the wounds in the photos.
%To perform TransMix, 
% material for pasting wounds.


%During training, for some images in a batch, we first found the position of the wound in the original images and then randomly selected wounds and pasted it on the same position as the original wound. The important thing to note here is that the wounds in the images have quite different sizes and aspect ratios. Therefore, when choosing which wounds to apply, we deliberately select those with not too significant differences in size compared to the original wound and then resize it to match the original size.
%
% To further enhance the reality and variability of synthesized photos. We will first remove the background of the wound patch based on the corresponding mask and then apply it to the original image. This can more effectively fit the applied wounds with the background of the original image and generate images that better match real-life situations. In addition, due to the removal of the background from the original image, coupled with the random selection of applied wounds, the variability of augmented wounds is significantly enhanced compared to the original. The enhanced wound variability also improve the performance of our model. 


% \subsubsection{Fine-tuning} 
% With the pre-trained model using the large-scale HAM10000 dataset, we fine-tune the model using 

%After pre-training our model on the HAM10000 dataset, we use the model as the initial weight in our fine-tuning phase. In this phase, the available data are limited despite that the degree of variation in the photos within the FUSeg dataset is quite significant, including factors such as shooting angle, shooting distance, and illumination conditions. To address this issue, we also perform strong transformations when fine-tuning to training a good model with limited data.\\
